Revisiting Robustness in Priced Timed Games

Priced timed games are optimal-cost reachability games played between two players---the controller and the environment---by moving a token along the edges of infinite graphs of configurations of priced timed automata. The goal of the controller is to reach a given set of target locations as cheaply as possible, while the goal of the environment is the opposite. Priced timed games are known to be undecidable for timed automata with $3$ or more clocks, while they are known to be decidable for automata with $1$ clock. In an attempt to recover decidability for priced timed games Bouyer, Markey, and Sankur studied robust priced timed games where the environment has the power to slightly perturb delays proposed by the controller. Unfortunately, however, they showed that the natural problem of deciding the existence of optimal limit-strategy---optimal strategy of the controller where the perturbations tend to vanish in the limit---is undecidable with $10$ or more clocks. In this paper we revisit this problem and improve our understanding of the decidability of these games. We show that the limit-strategy problem is already undecidable for a subclass of robust priced timed games with $5$ or more clocks. On a positive side, we show the decidability of the existence of almost optimal strategies for the same subclass of one-clock robust priced timed games by adapting a classical construction by Bouyer at al. for one-clock priced timed games.

==> 1ptg-new.tex <==
In this section, we define some subclasses of 1-clock PTGs.
Let $x$ denote the single clock that is used, and 
let $M$ be  the bound on the value $x$ can assume.   
This is ensured by explicit constraints that reset $x$ 
whenever $x$ reaches $M$. 



    


==> 1ptg.tex <==
In this section, we define some subclasses of 1-clock PTGs.
Let $x$ denote the single clock that is used, and 
let $M$ be  the bound on the value $x$ can assume.   
This is ensured by explicit constraints that reset $x$ 
whenever $x$ reaches $M$. 
A cycle is reset-free if the clock $x$ is not reset in the cycle.

A cycle $s_0 s_1 \dots s_0$ is non-blocking iff 
$(s_0 s_1 \dots s_0)^{\omega}$ is a valid run.\footnote{Note that 
 a cycle consisting of locations $s_0, s_1$ and guards $0<x<1$ from $s_0$ to $s_1$ 
  and $1<x<2$ from $s_1$ to $s_0$ is blocking.}
We assume henceforth that all cycles are non-blocking. 
A reset-free cycle $s_0s_1 \dots s_0$ is negative  
if (1) it has no precise constraints of the form 
$x=c$\footnote{Precise constraints, in the absence of resets,
mean no time elapse after the first iteration of the cycle.}
        on any of the transitions forming the cycle, and (2)
the cost accumulated in the first iteration of the cycle is negative. 
%Thus, any negative cycle can only have constraints of the form $x<1$.
The ``no reset'' condition ensures that further iterations of the cycle $(s_0s_1 \dots s_0)^i$ for $i > 0$ have no effect 
on the cost accumulated : if the cost accumulated in the first iteration $s_0 \dots s_0$ is negative, it will stay 
negative; likewise it will stay positive if the cost accummulated in the first iteration was positive.   
Note that a reset-free negative cycle is zeno. 
A  cycle $s_0 \dots s_0$ is non-zeno negative if the clock $x$ is reset 
on the cycle, and the accumulated cost on any iteration of $s_0 \dots s_0$ is  negative.
We denote by $\ZPTG{}$ the class of 1-clock PTGs which does not have any non-zeno negative
cycles: all cycles in this PTG are either  non-negative cycles or zeno
negative cycles.   
We denote by \NZPTG{} the class of all  1-clock PTGs which has atleast one non-zeno
negative cycle. 
We denote by \PTGP{} the class of all 1-clock PTGs which has only non-negative
prices. 
%\begin{corollary}
%\label{patcor}
%In an acyclic 1-clock PTG, both players have  
 %$\epsilon-$optimal memoryless strategies.
%\end{corollary}
%\begin{proof}
%Consider an acyclic 1-clock PTG $\ptg$. It is easy to see that the 
%classical attractor analysis on the underlying untimed graph would 
%prescribe the transition choice of any strategy $\strat$. 
%On this 1-clock PTG $\ptg$, we can apply all the transformations 
%considered in \cite{BouLar06} : (1) bounding the clock to be between 0 and 1, and (2) 
%transforming it into a reset-free PTG.   The reset-free PTG so obtained in  
%\cite{BouLar06} had only negative slopes 
%which are continuous and piece-wise affine 
%at all locations since the prices were non-negative. 
%The optcost of each location $l$ was computed by superimposing 
%the cost functions of the successors
%of $l$ and taking the exterior or the interior depending on whether $l$ is a player 2 or a player 1 location. 
%The only change in our case is that the slopes can be positive since we allow negative prices; however,
 % the optcost computation is not affected by this.  However, we wish to highlight that 
%the reason \cite{BouLar06} does not hold in the presence of cycles with an example in Figure \ref{fig:counterEx}. 
%\input{./figs/robust-counterEx.tex}
%\end{proof}

\begin{lemma}
 \label{lem:no_loop}
Let  $\zptg$ be a $\ZPTG$.
Then player 1 does not benefit by any strategy that revisits a location.  
  \end{lemma}
\begin{proof}
 Player~1's objective is to reach a target while minimizing the cost accumulated. Due to his objective to reach a target, he has no incentive in visiting a location again, provided it does not reduce the cost. There are four kinds of cycles : non-zeno positive cycles, zeno positive cycles, zeno negative cycles and non-zeno negative cycles. 
 A non-zeno negative cycle is the only one which can reduce the cost of a play;  since the PTG does not have such cycles, player 1 will never re-visit a location. 
However, if Player~2 can ensure that any cycle is taken, then he will stay in the cycle forever (and thus never reach a target). Hence it can not be a winning play for Player~1. Hence, a play that is winning for Player~1 in a  $\ZPTG$ never has a loop.
\end{proof}
%Note that Lemma \ref{lem:no_loop} will not hold 
%in the presence of discrete edge costs. If the zeno-negative cycle has 
%atleast one transition cost $p<0$ then Player~1 will want to take this cycle again and again 
%even though no time elapses as the cost of the play keeps reducing with each loop through the cycle. 
%However, if all of the transition costs in the zeno-cycle are $\geq 0$ then the Lemma \ref{lem:no_loop}  will continue to hold. 


==> ccp.tex <==
% A $\Sigma$-labeled graph is a tuple $S {=} (N, E, \preceq, L)$ where $N$ is
% a finite set of nodes,  $E \subseteq N \times N$ is a set of edges, $\preceq
% \subseteq N \times N$ is transitive closure of $E$, and $L: N \to \Sigma$ is a
% node-labeling function.       
% Let $GR(\Sigma)$ be the set of all $\Sigma$-labeled graphs.



% \subsection{Aperiodic Streaming String Transducers}
% Given a non-deterministic streaming string transducer 
% $T = (\Sigma, \Gamma, Q, q_0, \delta, X, \rho, F)$, we define its
% \emph{transition monoid}. 
% Wlog we assume that there exists a variable
% $o\in X$ such that $\rho(q,a)(o) = o$ for all $q\in Q$ and $a\in \Sigma$. 
% Let $w\in \Sigma^*$, and suppose that there exists a run $r$ from some state $p$
% to some state $q$ on $w$. Remind that this run induces a substitution $\sigma_r$.
% For all $x,y\in X$ such that $y$ occurs in $\sigma_r(x)$, we say that 
% \emph{$y$ $r$-flows to $x$}. For all states $p,q\in Q$ and strings $s\in\Sigma^*$, we say that
% \emph{$(p,y)$ flows to $(q,x)$ on $w$}, denoted by $(p,y)\rightsquigarrow^s (q,x)$, if there exists a run $r$ of $T$ on $s$ from state $p$
% to state $q$ such that $y$ $r$-flows to $x$. We say that $y$ flows to $x$ on $s$, denoted by 
% $y\rightsquigarrow^s x$ if there exist $p,q\in Q$ such that $(p,y)\rightsquigarrow^s (q,x)$.


% The \emph{transition monoid} of $T$ is defined as the set of $|Q|\times |X|$-square Boolean matrices
% $M_T = \{ M_s\ |\ s\in \Sigma^*\}$ where for all strings $s\in \Sigma^*$, $M_s[p,y][q,x] = 1$ iff
% $(p,y)\rightsquigarrow^s (q,x)$. 




% \begin{lemma}
% $(M_T,\times, 1)$ is a monoid, where $\times$ is defined as matrix multiplication and 
% $1$ is the unit matrix.  
% % Let $\Phi$ be the mapping defined as $\Phi(w) = M_w$ for all $w\in\Sigma^*$. Then $\Phi$ is
% % a morphism from $(\Sigma^*, ., \epsilon)$ to $(M_T, \times, 1)$. 
% \end{lemma}



% % \begin{proof}
%     % Clearly, $\Phi(\epsilon) = 1$. It is also clear that $\Phi(w.w') = \Phi(w)\times \Phi(w')$, i.e.
%     % $M_{w.w'} = M_w\times M_{w'}$ (left as an exercise). 
% % \end{proof}

% % We say that $M_T$ is \emph{aperiodic} if there exists $m\in\mathbb{N}$ such that 
% % for all $x\in M_T$,\ $x^m = x^{m+1}$. 
% An \nsst{} $T$ is called \emph{aperiodic} if its transition
% monoid is. The class of aperiodic \nsst{} is denoted by $\nast$ while the class of aperiodic
% deterministic \sst{} is denoted by $\ast$. 



==> contrib.tex <==
While the technique we have used closely resembles that of \cite{BouLar06}, 
we believe we have made  significant contributions to this work. 
We now list our contributions to this problem - 
\begin{enumerate}
 \item 	the first transformation RPTG to PTG : very careful and elegantly captures the robust seantics
 \item 
\end{enumerate}


==> proof_resetfree_frptg_old.tex <==
% We shall thus focus our energy on establishing that fractional resets do not break that proof. 
% 
% A fractional reset is taken only from a $[\delta,2\delta]$-delay location. This is a Player~2 location 
% and is created in the PTG to simulate Perturbator actions. Thus, a fractional reset will result in a 
% state $(l,\val) \xrightarrow{\fr{x}}(l',frac(\val))$ where $frac(\val)\in [0,\delta]$ due to the delay 
% restriction on $l$. A fractional reset does not give us the special property of visiting the same state 
% again (as the case with a reset). However, we continue to argue that the technique in \cite{BouLar06} 
% extends even in the presence of fractional resets. Here is our logic : 
% 
% We believe there is nothing very sacrosanct about a fractional reset apart from the fact that it jumps from one 
% location to another and retains the fractional part.. now the labels of the locations have registered 
% the fact the integer part switched to the next number. Now, the important point I want to stress is the following : 
% the fractional part carried over is in the interval of $[0,\delta]$ \todom{We are losing the solution to 
% general \FRPTG}. Also, our outside cost functions and optcost functions computed are over the domain $[0,1+\delta]$. 
% So, even when the valuation crosses 1 in the \FRPTG which is meant to bound the clock to $[0,1]$, 
% we do not make the outside cost functions invalid or undefined. 

\noindent We now discuss the usefulness of the fractional resets. 
Recall that  we wanted to bound the clock strictly to $[0,1]$ at all the original locations 
of the RPTG, which are not present in the converted PTG. 
The delay that the perturbator intended to spend at $\posP{l,e}$ (before bounding) was $t = \delta+\alpha$ where $\delta$ of it to compensate for Player~1 choosing $d-\delta$ in the $\delta$-dwell-time PTG $\ptg$ as opposed to $d$ in the RTG $\rtg$. Here $\alpha$ is his actual positive perturbation.
Let us try to model this without using fractional resets. 
 
   Assume that we split this time delay $t$ into $t_1$ and $t_2$ such that $\val+t_1 =1$, 
where $\val$ is the valuation 
with which the location $\posP{l,e}$ is entered in the $\delta$-dwell-time PTG $\ptg$.
 Let us construct a PTG with two locations such that the total time elapse 
 across these locations is $t$.    Let us denote this PTG as  $\ptg_N$. 
    The PTG $\ptg_N$ where $t_1$ and $t_2$ are split across the two locations $\posP{l,e}_i$ and $\posP{l,e}_{i+1}$  is shown in the figure below.  
     However, such a split will mean that we do not know a priori what $t_1$ and $t_2$ will be as they depend on $\val$. 
 The optcost computation is done location wise, by superimposing the cost functions 
   of the successors of any location, and computing the interior or exterior depending on the nature 
   of the location. In the PTG $\ptg_N$, from the optcost computations 
   for the locations with time delay $t_1, t_2$, we cannot ensure that 
   $t_1+t_2 \in [\delta, 2 \delta]$, since this information is split across two locations 
   and the optcost computation is handled location wise. 
     Thus, while it looks difficult to  solve the PTG $\ptg_N$\footnote{Since in the \FRPTG, the time delay is at the single location, the optcost computation us easier.}, 
     such a PTG would help us establish the equivalence of the \FRPTG~ with the resetfree \FRPTG :
since the PTG $\ptg_N$ has no fractional resets, the transformation in \cite{BouLar06}, wherein 
a reset-free game graph is obtained is applicable to $\ptg_N$, and 
the equivalence of the $\ptg_N$ and its reset-free counter part can be shown 
as in \cite{BouLar06}. \\~\\

\input{./figs/fr_proof.tex}

It is obvious that $\ptg_N$ has more behaviors than $\frptg$, since 
by construction of  $\ptg_N$, we have 
$t_1+t_2 \in[0,1+\delta]$ in PTG $\ptg_N$ (a maximum amount of 1 time unit can be spent at 
$\posP{l,e}_i$ and $\delta$ time at $\posP{l,e}_{i+1}$). 
  We can restrict this 
time to lie in the interval $[\delta, 2\delta]$ by putting a dwell-time restriction on $\ptg_N$. 
Let us now consider $\ptg_N$ to be a dwell-time PTG, which has the dwell time restriction 
  that  $t_1+t_2 \in [\delta,2\delta]$.  
  \begin{lemma}
  \label{lem:NandFR}
  The dwell-time PTG $\ptg_N$ preserves the optcost of 
the $\delta$-dwell-time PTG $\ptg$ obtained from the original RPTG. 
Further, its  optcost is also equivalent to that of the FRPTG $\frptg$.
  \end{lemma}
  \begin{proof}
  In the FRPTG $\frptg$, the transition from the location $\overline{(l,e)_i}$  to the location 
  $\overline{(l,e)_{i+1}}$ results in $x$ having a value in $[0, \delta]$, since 
  a time delay in the interval $[\delta, 2 \delta]$ is possible at  $\overline{(l,e)_i}$.
  Entry into $\overline{(l,e)_i}$ happens with $x \leq 1-\delta$, and the integer part 1 is removed on entering 
  $\overline{(l,e)_{i+1}}$, resulting in $x$ having a value in $[0, \delta]$. 
  $\overline{(l,e)_{i+1}}$ is urgent, and hence we reach $C$ with $x \in [0, \delta]$.
    Note that in the PTG $\ptg_N$ also, 
  we enter $\overline{(l,e)_{i}}$ with the same value of $x$ as in the FRPTG (that is, $x \leq 1-\delta$).
  Since at most $\delta$ delay happens at $\overline{(l,e)_{i+1}}$ in $\ptg_N$, we obtain the value of $x$ in 
  $[0, \delta]$ at $C$.  The proof follows since the time delay spent by player 2 
  at $\overline{(l,e)_{i+1}}$ in the FRPTG can be mapped to the total time delay spent by the two player 2 locations  
  $\overline{(l,e)_{i}}$ and $\overline{(l,e)_{i+1}}$ in the PTG $\ptg_N$ and vice-versa.   
  \end{proof}
  
  
  Now, the crucial property of this dwell-time  PTG $\ptg_N$ is that it does not have fractional resets:  a resetting transition taken twice, hence takes us back to the same state twice. This crucial property is the back bone of the transformation which removes resets in \cite{BouLar06}. 
Hence, it can be shown that this dwell-time PTG $\ptg_N$ is equivalent 
to its reset-free counterpart (similar to \cite{BouLar06}). 
\begin{lemma}
\label{lem:NandFR_r}
  The reset-free dwell-time PTG $\ptg'_N$ preserves the optcost of 
the reset-free-FRPTG $\frptg'$.
  \end{lemma}
  \begin{proof}
  The proof of this Lemma is similar to that of Lemma \ref{lem:NandFR}. 
  When we construct the reset-free FRPTG, from the given FRPTG,  
  a new component is created each time  a fractional reset between 
  $\overline{(l,e)_{i}}$ and $\overline{(l,e)_{i+1}}$ happens.  
    Corresponding to this, 
    a new component is created by the reset transition between locations 
  $\overline{(l,e)_{i}}$  and $\overline{(l,e)_{i+1}}$, in the reset-free PTG corresponding to  
  PTG $\ptg_N$. The argument in Lemma \ref{lem:NandFR} therefore 
  applies here as well; whenever a new component is created in the reset-free FRPTG 
  after a delay $t \in [\delta, 2\delta]$ at $\overline{(l,e)_{i}}$,  a new component
  is created in the reset-free PTG $\ptg_N$ from the location $\overline{(l,e)_{i}}$  after a 
  delay $t_1$; however the starting location $\overline{(l,e)_{i+1}}$
  of this new component incurs a time delay $t_2$ such that 
  $t_1+t_2=t$.
 \end{proof} 

\input{./figs/resetfree_proof.tex}

We thus have 
\begin{enumerate}
\item $\ptg_N$ preserves the opt cost of the $\delta$-dwell-time PTG $\ptg$, (Lemma \ref{lem:NandFR}) 
\item $\ptg_N$ preserves the opt cost of the FRPTG obtained from $\ptg$, (Lemma \ref{lem:NandFR})
\item  The reset-free counter part $\ptg'_N$ of $\ptg_N$ 
preserves the optcost of $\ptg_N$~\cite{BouLar06}, 
\item $\ptg'_N$ preserves the optcost of 
 $\frptg'$ (Lemma \ref{lem:NandFR_r})
\item The points above show that the reset-free counter part $\frptg'$ of the 
$\FRPTG$ $\frptg$ preserves the optcost of $\frptg$.  
\end{enumerate}

Figure \ref{flow} gives the entire flow of reductions. 
We thus obtain the equivalence between the optcost
of the $\FRPTG$ $\frptg$ and its reset-free counter part $\frptg'$.
Hence, the following lemma holds.

\begin{lemma}
 \label{lem:resetfree_frptg}
 For every state $(l,\val)$ in $\frptg$, $\optcost{\frptg}(l,\val) = \optcost{\frptg'}(l^0,\val)$, where  
 $\frptg'$ is the resetfree \FRPTG. For every $\epsilon >0, N \in \Nat$, given an $(\epsilon,N)$-acceptable strategy $\sigma'$ in $\frptg'$, we can compute a $(2\epsilon,N)$-acceptable strategy $\sigma$ in $\frptg$ and vice versa.
\end{lemma}
\begin{proof}
Consider any state $(l, \val)$ in $\frptg$.  The reduction from 
the FRPTG $\frptg$ to the reset-free 
FRPTG $\frptg'$  
creates a new component (or copy) for each new reset, including fractional resets.
Given that there are a total of $n$ resets in the FRPTG, 
$\frptg$, $n+1$ reset-free components are created in the reset-free FRPTG 
$\frptg'$, and the last component goes to a location with cost $+\infty$. 
By assumption, the cycles in each reset-free component 
are non-negative.   As seen in Lemma \ref{lem:no_loop}, 
player 1 does not benefit by revisiting a state, while player 2 
will always choose a loop whenever possible. 
Any cycle in the FRPTG $\frptg$ involving a reset 
is mapped to a path in the reset-free FRPTG $\frptg'$ ending at the location $S$ with cost $+\infty$, 
while any reset-free cycle in $\frptg$ is mapped to  a  cycle 
in one of the $n+1$ reset-free components of the reset-free FRPTG $\frptg'$. 
Clearly, for every strategy $\sigma$ of player 1, 2 in $\frptg$, there is a corresponding strategy $\sigma'$ in the 
$\frptg'$ and vice-versa,  obtained using the above mapping of paths 
between $\frptg$ and $\frptg'$.  Given that the prices of locations are preserved between 
$\frptg$ and $\frptg'$, the optimal cost from $(l, \val)$ in 
$\frptg$ is the same as the optimal cost from $(l^0, \val)$ in $\frptg'$. 


%Consider a $(\epsilon,N)$-acceptable strategy $\sigma'$ in $\frptg'$. 
%Consider any state $(l, \nu)$ in $\frptg$. Assume that $i$ is the minimum number of resets 
%required on any path from $(l, \nu)$ to reach a target state, compatible with $\sigma$. 
%Correspondingly, we have in $\frptg'$, a path from $(l^{n-i}, \nu)$ 
%reaching  a target state, but no path from   $(l^{n-i+1}, \nu)$
%to a target state. Also, we have for any $(\epsilon,N)$-acceptable strategy $\sigma'$ in $\frptg'$, it cannot be the case that  
%$\costp_{\frptg'}((l^{n-i},\nu), \sigma') > \costp_{\frptg'}((l^0, \nu), \sigma')+\epsilon$.
%That is, $\costp_{\frptg'}((l^{n-i},\nu), \sigma') \leq \costp_{\frptg'}((l^0, \nu), \sigma')+\epsilon$.
%   We thus have $\costp_{\frptg'}((l^{n-i},\nu), \sigma') \leq \optcost{\frptg'}((l^{n-i},\nu))+\epsilon \leq 
%\optcost{\frptg'}((l^0,\nu))+\epsilon +\epsilon$.

Consider a $(\epsilon,N)$-acceptable strategy $\sigma'$ in $\frptg'$. Consider a winning state $(l^0,\nu)$. Let $i$ be the minimum number of resets 
from state $(l^0,\nu)$ along any path compatible with $\sigma'$. That is, the player can win from $(l^{n-i},\nu)$ but not from $(l^{n-i+1},\nu)$. If $(l,\nu)$ is not winning then we take $i=n+1$. We denote by $\sigma'_{n-i}$ the suggestions made by $\sigma'$ in the $n-i^{th}$ copy in $\frptg'$. We  then assign $\sigma(l,\nu) = \sigma'_{n-i}(l^{n-i},\nu)$. Thus, we obtain that $\costp_{\frptg}((l,\nu),\sigma) = \costp_{\frptg'}((l^{n-i},\nu),\sigma')$. 
We know that 
\begin{equation}\label{eqn1}
 \costp_{\frptg'}((l^0,\val),\sigma') \geq \optcost{\frptg'}(l^{n-1},\val)
\end{equation}
Now, if $\costp_{\frptg'}((l^{n-i},\nu),\sigma') ~> ~\costp_{\frptg'}((l^0,\nu),\sigma') + \epsilon$, then by Equation \ref{eqn1} we 
have $\costp_{\frptg'}((l^{n-i},\val),\sigma')>\optcost{\frptg'}(l^{n-i},\val)+\epsilon$ which means $\sigma'$ is not $\epsilon$-optimal. Thus we have, 
$\costp_{\frptg}((l,\nu),\sigma) = \costp_{\frptg'}((l^{n-i},\nu),\sigma') $ \\
$\costp_{\frptg'}((l^{n-i},\nu),\sigma') ~\leq ~\costp_{\frptg'}((l^0,\nu),\sigma') + \epsilon$
\begin{equation*}
\costp_{\frptg}((l,\nu),\sigma)
    \begin{cases}
		\leq ~\costp_{\frptg'}((l^0,\nu),\sigma') + \epsilon \\    
		\leq~\optcost{\frptg'}(l^0,\nu) + \epsilon + \epsilon \\
		\leq~\optcost{\frptg}(l,\nu) + 2\epsilon
    \end{cases}
\end{equation*}

  







  

  
      








\end{proof}

==> robust-main.tex <==
\part{Robustness}

%\chapter*{Part 3 : Robustness}
%\addcontentsline{toc}{chapter}{\Large{\textbf{Part 3 : Robustness}}}
  
\chapter{Robust Priced Timed Games}
\label{chap:robust}

\input{abstract.tex}
\section{Introduction}
\label{sec:robust-intro}
\input{robust-intro.tex}

\section{Preliminaries}
\label{sec:prelims}
\input{robust-ptg_syntax.tex}

\section{Robust Semantics}
\label{sec:robust-prelims}
\input{robust-prelims.tex}


\section{Decidability with 1 clock}
\label{sec:robust-dec}
\input{robust-dec1clk.tex}

 \section{Undecidability with 5 clocks}
 \label{sec:robust-undec}
 \input{robust-undec_excess_nonGame.tex}


 \section{Conclusion and Future Work}
 \label{sec:robust-concl}
 \input{robust-conclusion.tex}
 
 


==> robust-prelims_old.tex <==
% \section{\bf Robust Semantics.}

%% In this section, we  define turn-based robust priced timed games. Concurrent 
%% robust priced timed games were studied in \cite{ocan}.
A Robust-PTG (RPTG) is a PTG where Player~1 is called controller and Player~2 is called the perturbator. 
The additional property is that perturbator can perturb (alter) the delay chosen 
by controller by an amount 
in $[-\delta, \delta]$, where $\delta>0$ is a pre-defined bounded quantity. 
Further, the time delay in all locations must be $\geq \delta$.
\cite{ocan} considered two kinds of perturbation semantics : 
(i) excess semantics, where the 
perturbation happens after the constraint is satisfied. The resets come into effect after the perturbation, 
(ii) conservative semantics,  where the constraint has to be satisfied 
after the perturbation.
We call an RPTG Robust-Priced Timed Automata (RPTA)\footnote{Note that our definition of RPTA coincides with that in \cite{ocan}, 
  while our RPTG are turn-based.} when perturbator does not explicitly control
any location. 
Thus, in an RPTA, all locations are controller locations, and, for a chosen
$\delta$, perturbator can perturb the time delays chosen by the controller.  
The excess perturbation as well as the conservative perturbation are defined 
in the same way as in the RPTG. 

%% Bouyer et al.~\cite{ocan} considered robust priced timed automata and games under 
%% both semantics, and studied the problem of deciding an upperbound 
%% on the limit cost of a winning strategy for reachability objectives 
%% of the controller. The limit-cost refers to the limit of the cost as $\delta$ 
%% tends to zero, that is when there are no perturbations. 
%% \cite{ocan} showed that the limit cost  reachability problem 
%% is undecidable for robust priced timed automata under the excess perturbation semantics, and 
%% undecidable for games under the conservative semantics. 
%% Decidability was obtained only for the case of robust priced timed automata 
%% under the conservative semantics. 
%% In this paper, we look closer into the 
%% excess perturbation semantics, and show that for a fixed $\delta$, the cost optimal 
%% reachability problem is decidable for 
%% 1-clock robust priced timed games 
%% having no negative cost cycles with a reset. We also improve the undecidability of the limit cost reachability problem 
%% under excess semantics to 5 clocks. 
\begin{definition}[Perturbation Semantics]
Given a $\delta>0$ the $\delta-$excess semantics of a Robust-PTG $\rtg$ is a LTS 
$\sem{\rtg}$ = $(\nSR,\nAR,\nTR)$
where $\nSR = \states_1 \cup \states_2$, $\nAR = \actions_1 \cup \actions_2$ and $\nTR =\nTR_1 \cup \nTR_2$. 
We define the set of states, actions and transitions for each player below. 
\begin{itemize}
\item $\states_1 = \locations_1 \times \V \times \C$ are the controller states,
% \todom{Remove $\C$ - cost valuation? from state defn}
\item $\states_2 = (\locations_2 \times \V \times \C) \cup (\states_1 \times \Rplus \times \trans)$ are the perturbator states, 
\item $\actions_1 = \Rplus \times \trans$ are controller actions
\item $\actions_2 = \Rplus \times \trans \cup [-\delta,\delta]$ are perturbator actions

\item $\nTR_1 = (\states_1 \times \actions_1 \times \states_2)$ is the set of 
controller transitions such that for a controller state $(l,\val,\cost)$ and a controller action $(t,e)$ we have 
$((l,\val,\cost),t,e)  = \nTR_1((l,\val,\cost),(t,e))$ iff there is a transition $e=(l,g,a,r,l')$ in $\rtg$ such that 
$\val + t \in \sem{g}$. 

\item $\nTR_2 = \states_2 \times \actions_2 \times (\states_1 \cup \states_2)$ is the set of perturbator transitions
such that for a perturbator state of the type $(l,\val,\cost)$ and a perturbator action $(t,e)$ we have 
$(l',\val',\cost')  = \nTR_2((l,\val,\cost),(t,e))$ iff there is a transition $e=(l,g,a,r,l')$ in $\rtg$ such that 
$\val + t \in \sem{g}$, $\val' = (\val + t)[r:=0]$ and $\cost' = \cost + \prices(l) * t$. 
\newline
For a perturbator state of type $((l,\val,\cost),t,e)$ and a perturbator action $\epsilon \in [-\delta,\delta]$ we have $(l',\val',\cost') = \nTR_2(((l,\val,\cost),t,e),\epsilon)$ iff 
\begin{itemize}
 \item $e = (l,g,a,r,l')$,
 \item $\val' = (\val + t + \epsilon)[r:=0]$, 
 \item $\cost' = \cost + \prices(l) * (t + \epsilon)$
\end{itemize}
\end{itemize}
\end{definition}
Note that these semantics are the excess semantics since we check  the satisfaction 
of the constraint before the perturbation 
and the transition; however, the  reset occurs after the perturbation. 
The delays chosen by the controller should be at least $\delta$ to ensure the 
system is not infinitely fast \cite{ocan}. 
The notions of a path and winning play are  same as in PTG. We shall now 
adapt the definitions of cost of a play, and a strategy for the excess perturbation semantics. 
Let $\rho$ $=s_1 \xrightarrow{t_1,e_1} s_2 \xrightarrow{t_2,e_2}\cdots \xrightarrow{t_{n-1},e_{n-1}}s_n$ be a path in the LTS $\sem{\rtg}$. 
Given a $\delta>0$, we define $\costp_{\rtg}^{\delta}(\rho) = c_n$ where $s_n = (l_n,\val_n,c_n)$. Also, we re-define the cost of a strategy $\strat_1$ from 
state $s$ for a given $\delta>0$ as $\costp_{\rtg}^{\delta}(s,\strat_1) 
 = \sup_{\strat_2 \in \maxstrats{\rtg}} \costp_{\rtg}^{\delta}(\outcome(s,\strat_1,\strat_2))$. Similarly, $\optcostd{\rtg}$ is the optimal cost 
 under excess perturbation semantics for a given $\delta>0$.
 $\optcostd{\rtg}(s) = $ 
$\inf_{\strat_1 \in \minstrats{\rtg}} \sup_{\strat_2 \in \maxstrats{\rtg}} (\costp^{\delta}(\outcome(s,\strat_1,\strat_2)))$.
  Since  optimal strategies may not always exist, 
 we define 
$\epsilon-$optimal strategies such that 
for every $\epsilon>0$, 
$\optcostd{\rtg}(s) \leq \costp_{\rtg}^{\delta}(s,\strat_1) < \optcostd{\rtg}(s)+\epsilon$. 

 
 
 Now, we shall define limit variations of costs, strategies and values as $\delta \rightarrow 0$. 
 The \emph{limit-cost} of a controller strategy $\sigma_1$ from  state $s$ 
 is defined as \\ ${\limcost}_{\rtg}(\strat_1,s) 
 = lim_{\delta \to 0}\sup \set{\costp_{\rtg}^{\delta}(\rho)\mid \rho \mbox{ starts from $s$ and is compatible with}\strat_1}$. Limit-cost is well defined as $\strat_1$ is valid 
 for any $\delta>0$. 
 The \emph{limit strategy upper-bound problem}\cite{ocan} for excess perturbation semantics asks, given a Robust-PTG $\rtg$, state $s=(l,\zero,\zero)$ and rational $K$, whether there exists 
 a strategy $\strat_1$ such that $\limcost_{\rtg}(\strat_1,s) \leq K$. 
  The following are the main results of \cite{ocan} with respect to the excess perturbation semantics.
 \begin{theorem}[Known results \cite{ocan}]
 \label{thm:robust_known}
\begin{enumerate}
 \item The limit-strategy upper-bound problem is undecidable for 
 RPTA and RPTG under excess perturbation semantics, for $\geq 10$  clocks.
  \item  For a fixed $\delta \in[0, \frac{1}{3}]$, 
 and a given RPTA $\rta$, a target location $l$ and a rational $K$, 
 it is undecidable whether  $\inf_{\strat_1} \sup_{\strat_2}cost_{\strat_1,\strat_2}(\rho) < K$ such that $\rho$ ends in $l$.
  $cost_{\strat_1,\strat_2}(\rho)$ is the cost of the unique run $\rho$ obtained 
  from the pair of strategies $(\strat_1, \strat_2)$.
% \todomr{Is this the same as $\optcostd{\rtg}(s)$ : but we are computing FROM $s$ where as this problem is TO a target.. however, we can solve this problem too with our optcost computations.. remove all targets other than $l$ and apply our technique.}
\end{enumerate}
 \end{theorem}
 
 We now list our main contributions in the following theorems. 
 
  \begin{theorem}
  \label{thm:robust_undec}
  The limit-strategy upper-bound problem is undecidable for RPTA with 5 clocks and prices $\set{0,1,-1}$.
 \end{theorem}

 
 \begin{theorem}
 \label{thm:robust_dec}
  Given a 1-clock RPTG $\rtg$ which has no negative cycle involving the reset of clock\footnote{Note that our results continue to hold for cycles whose accumulated cost is negative, and which have no resets}  
  and a $\delta>0$, $\optcostd{\rtg}(s)$ for every state $s=(l,\val,0)$ is 
  computable. For every $\epsilon >0$ there exists an $N \in \Nat$ such that the controller 
 has an $(\epsilon,N)$-acceptable strategy.  
 \end{theorem}
 Note that Theorem \ref{thm:robust_dec} also shows that we can solve the following threshold problem : 
  for a fixed $\delta$, given a 1 clock RPTA, an initial location and a target location, 
 and a rational number $K$, 
is $\inf_{\strat_1} \sup_{\strat_2}cost_{\strat_1,\strat_2}(\rho) < K$? 

\begin{theorem}
 \label{thm:ptg_neg_cycle}
%  Given a 1 clock $\ptg$ with arbitrary prices and which has no negative cycle involving the reset of clock, 
Given a $\ZPTG$, 
 $\optcost{\ptg}(s)$ for every state $s$ is computable. For every $\epsilon >0$ there exists an $N \in \Nat$ such that Player~1 
 has an $(\epsilon,N)$-acceptable strategy.  
\end{theorem}
The proof follows from Theorem \ref{thm:robust_dec}. 
 




==> robust-ptg.tex <==
% 
\input{robust-abstract.tex}

\section{Introduction}
\label{sec:robust-intro}
\input{robust-intro.tex}

\section{Preliminaries}
\label{sec:robust-prelims}
\input{robust-ptg_syntax.tex}
\input{robust-prelims.tex}


\section{1 Clock Decidability}
\label{sec:robust-dec}
\input{robust-dec1clk.tex}


\section{Undecidability}
\label{sec:robust-undec}
\input{robust-undec_excess_nonGame.tex}

\bibliographystyle{plain}
\bibliography{papers_combined}


==> robust-ptg_syntax_1.tex <==
We write $\Real$ for the set of reals and $\Int$ for the set of integers.
Let $\pclocks$ be a finite set of real-valued variables called \emph{clocks}. 
A \emph{valuation} on $\pclocks$ is a function $\nu : \pclocks \to \Real$.
We assume an arbitrary but fixed ordering on the clocks and write $x_i$
for the clock with order $i$. 
This allows us to treat a valuation $\nu$ as a point $(\nu(x_1), \nu(x_2),
\ldots, \nu(x_n)) \in \Real^{|\pclocks|}$. 
Abusing notations slightly, we use a valuation on $\pclocks$ and a point in
$\Real^{|\pclocks|}$ interchangeably. 
For a subset of clocks $X \subseteq \pclocks$ and valuation $\nu \in \V$, we
write $\nu[X{:=}0]$ for the valuation where $\nu[X{:=}0](x) = 0$ if $x \in X$, and
$\nu[X{:=}0](x) = \nu(x)$ otherwise.
The valuation $\zero \in \V$ is a special valuation such that
$\zero(x) = 0$ for all $x \in \pclocks$.
A clock constraint over $\pclocks$ is a subset of $\Real^{|\pclocks|}$.
We say that a constraint is \emph{rectangular} if it is defined as the
conjunction of a finite set of constraints of the form 
$x  \bowtie k,$  where $k \in \Int$, $x \in \pclocks$, and $\bowtie \in \{<,\leq, =,
 >, \geq\}$.    
 For a constraint $g \in \rect(\pclocks)$, we write $\sem{g}$ for the set of valuations in
 $\Real^{|\pclocks|}$ satisfying the constraint $g$.  
 We write $\rect(\pclocks)$ for the set of rectangular constraints over
 $\pclocks$.
%
\begin{definition}[Priced Timed Games]
  A turn-based two player \emph{priced timed game} is a tuple
  $\ptg = (\locations_1,\locations_2, L_{init}, \pclocks, \trans, \prices,\rgoals)$ where 
    \begin{itemize}
    \item 
  $\locations_i$ is a finite set of \emph{locations} of Player~$i$, 
   \item 
  $L_{init} \subseteq L_1 \cup L_2$ is a set of initial locations,
    \item 
  $\pclocks$ is an (ordered) set of \emph{clocks}, 
   \item
  $\trans \subseteq \locations \times {\rect}(\pclocks)  \times 2^{\pclocks}
  \times \locations$ 
  is the \emph{transition relation}, 
    \item 
  $\prices \colon \locations \rightarrow \Z$ is the price
  function; and
    \item 
  $\rgoals \subseteq \locations$ is the set of target locations.
   \end{itemize}
\end{definition}

Note that for the sake of simplicity we have omitted the set of actions and location 
invariants from the definition of a PTG (included in definition of PTG in Chapter \ref{chap:ptg}). 
However, all of our results in this chapter hold in the presence of actions and invariants too. 


A priced timed game begins with a token placed on some initial location $\ell$ with  
valuation $\zero$ and cost accumulated being so far being $0$.  
At each round, the player who controls the current location $\ell$ chooses a delay
$t$ (to be elapsed in  $l$) and an outgoing transition $e =(\ell, g, r, \ell') \in
\trans$ to be taken after $t$ delay at $\ell$. 
The clock valuation is then updated according to the delay $t$ and
reset and the cost is incremented by $\prices(\ell) \cdot t$ and the token is moved 
to the location $\ell'$.   
The two players continue moving the token in this fashion, and give rise to a
sequence of locations and transitions called a \emph{play} of the game. 
A configuration or state of a PTG is a tuple $(\ell, \val, \cost)$ where $\ell \in
\locations$ is a location,  $\val \in \V$ is a valuation, and  $\cost$ is the
cost accumulated from the start of play.

W.l.o.g~\cite{BFHLPRV01} we assume that the clock values are bounded : there
exists an constant $M$ such that  $x \leq M$ is satisfied always for all $x \in \pclocks$. 

\begin{definition}[PTG semantics]
The semantics of a PTG $\ptg$ is a labelled state-transition game arena 
$\sem{\ptg}$ = $(\nSR = \states_1 \uplus \states_2, S_{init}, A, \nTR)$
where 
\begin{itemize}
\item 
  $\states_j = \locations_j \times \V $ are the Player~$j$ states with 
  $\nSR = \states_1 \cup \states_2$, 
\item 
  $S_{init} \subseteq \nSR$ are initial states s.t. $(\ell, \nu)
  \in S_{init}$ if $\ell \in L_{init}$, $\nu = \zero$ and $c = 0$,
\item 
  $A = \Rplus \times (\locations \times {\rect}(\pclocks)  \times 2^{\pclocks}
  \times \locations)$ is
  the set of \emph{timed moves}, and 
\item
  $\nTR: \nSR \times A \to \nSR$ is the transition function s.t. 
  for $s = (\ell, \nu), s' = (\ell', \nu') {\in} \nSR$ and
  $ \tau = (t, e) \in A$ the function $\nTR(s, \tau)$ is defined if $ e = (\ell, g, r,
  \ell')$ is a transition of PTG and $\nu \in \sem{g}$;
  moreover $\nTR(s, \tau) = s'$ if $\nu' = (\nu+t)[r{:=}0]$. 
  We write $s \xrightarrow{\tau} s'$ when $\nTR(s, \tau) = s'$.
\end{itemize}
%% The transition relation is defined as 
%% \begin{enumerate}
%% \item (discrete transition) $(l, \nu, c) \xrightarrow{e} (l', \nu', c')$ if there exists $(l, g,r,l') \in \trans$
%% such that $\nu \models g$, $\nu'=\nu[r{:=}0]$ and $c'=c$,
%% \item (delay transition) $(l, \nu, c) \xrightarrow{t} (l,  \nu',c')$ if 
%% $\nu'=\nu+t$, $c'=c+t\prices(l)$.
%\end{enumerate}
%We define the set of states  and transitions for each player below. 
%\begin{itemize}
%\item 
%\item 
%$\states_j = \locations_j \times \V \times \C$ are the Player~$j$ states, 
%\item $\actions_j = \Rplus \times \trans$ are the actions, 
% \item $goals' = \rgoals \times \V \times \C$
%\item 
%$\trans_j$ is the set of 
%Player~$j$ transitions.
%\end{itemize}
\end{definition}
%% For a  state $(l,\val,\cost)$ a pair $(t,e)$, we have 
%% $(l',\val',\cost')  = \nTR((l,\val,\cost),(t,e))$ iff there is a transition $e=(l,g,a,r,l')$ in $\ptg$ such that 
%% $\val + t \in \sem{g}$, $\val' = \val+t[r:=0]$ and $\cost' = \cost + \prices(l) * t$.

For a state $s = (\ell, \nu)$ we write $s(\ell)$ and $s(\nu)$ for the
location and valuation of the state. 

A \emph{play} $\rho = \seq{s_0, (t_1, a_1), s_1, (t_2, a_2), \ldots, s_n}$ is a
finite sequence of states and actions s.t.  $s_0 \in S_{init}$ and $s_i
\xrightarrow{(t_{i+1}, a_{i+1})} s_{i+1}$ for all $0 \leq i < n$.
For a finite play $\rho$ we write its last state as $\last(\rho) = s_n$. 
We denote the set of plays as $\runs_{\ptg}$. 
For a play  $\rho = \seq{s_0, (t_1, a_1), s_1, (t_2, a_2), \ldots, s_n}$ we define
$\costp_{\ptg}(\rho) = \sum_{i{=}0}^{n} t_i * \prices(s_{i-1}(\ell))$. 
A \emph{strategy} of player $j$ in $\ptg$ is a function $\strat : \runs_{\ptg}
\to A$ such that for a play $\rho$ the function $\strat(\rho)$  is defined if
$\last(\rho) \in \states_j$.  
We say that a strategy $\strat$ is memoryless if $\strat(\rho) = \strat(\rho')$
when $\left(\last(\rho)(\ell), \last(\rho)(\nu)\right) =
\left(\last(\rho')(\ell), \last(\rho')(\nu)\right)$, otherwise we call it
memoryful. 

We write $\mminstrats$ and $\mmaxstrats$ for the set of strategies of player $1$ and
$2$, respectively. 
A play $\rho$ is said to be \emph{compatible to a strategy} $\strat$ of player
$j \in \set{1, 2}$ if for every state $s_i$ in $\rho$ that belongs to Player~$j$,   
$s_{i+1} = \strat(s_i)$. 

Given a pair of strategies $(\sigma_1, \sigma_2) \in \mminstrats \times
\mmaxstrats$, and a state $s$,  the outcome of $(\sigma_1, \sigma_2)$ from
$s$ denoted  $\outcome(s, \strat_1, \strat_2)$ is the unique play that is
compatible with both strategies.  
Given a player $1$ strategy $\sigma_1 \in \mminstrats$ we define its cost
$\costp_{\ptg}(s,\strat_1)$  as 
$\costp_{\ptg}(s,\strat_1) \rmdef \sup_{\strat_2 \in
  \mmaxstrats}(\costp(\outcome(s,\strat_1,\strat_2)))$. 
%Similarly, we also introduce $\costp_{\ptg}(s,\strat_2)$ as the cost of a Player~2 strategy. 
We now define the  \emph{optimal reachability-cost} for Player~1 from a state
$s$ as 
\[
\optcost{\ptg}(s) = \inf_{\strat_1 \in \mminstrats} \sup_{\strat_2 \in
  \mmaxstrats} (\costp(\outcome(s,\strat_1,\strat_2))).
\]  
A strategy $\strat_1 \in \mminstrats$ is said to be optimal from $s$ if 
$\costp_{\ptg}(s,\strat_1) = \optcost{\ptg}(s)$. 
Since  the optimal strategies may not always exist~\cite{BouLar06} we define the
concept of $\varepsilon$ optimal strategies. 
For $\varepsilon  > 0$ a strategy $\sigma_\varepsilon \in \mminstrats$
is called $\varepsilon-$optimal if  
\[
\optcost{\ptg}(s) \leq \costp_{\ptg}(s,\strat_\varepsilon) < \optcost{\ptg}(s)+\varepsilon.
\] 
The \emph{cost-optimal} reachability problem for PTG asks : given a PTG $\ptg$
and a bound $K \in \Z$ decide whether there exists a strategy for player~1 such
that $\optcost{\ptg}(s) \leq K$ for some starting state $s$. 
The following is a well known result.
\begin{theorem}[\cite{BouBri06}]
  The cost-optimal reachability problem is undecidable for priced timed automata
  with $3$ or more clocks. 
\end{theorem}
\begin{theorem}[\cite{BouLar06,DueIbs13,Rut11}]
\label{thm:1ptg_pat}
  For one-clock priced timed games, the problem of computing
  $\varepsilon$-optimal strategy is decidable.
\end{theorem}



\paragraph{\bf One-Clock PTGs.}

\input{1ptg}


==> robust-ptg_syntax_old.tex <==
We write $\Real$ for the set of reals and $\Int$ for the set of integers.
Let $\clocks$ be a finite set of real-valued variables called \emph{clocks}. 
A \emph{valuation} on $\clocks$ is a function $\nu : \clocks \to \Real$.
We assume an arbitrary but fixed ordering on the clocks and write $x_i$
for the clock with order $i$. 
This allows us to treat a valuation $\nu$ as a point $(\nu(x_1), \nu(x_2),
\ldots, \nu(x_n)) \in \Real^{|\clocks|}$. 
Abusing notations slightly, we use a valuation on $\clocks$ and a point in
$\Real^{|\clocks|}$ interchangeably. 
For a subset of clocks $X \subseteq \clocks$ and valuation $\nu \in \V$, we
write $\nu[X{:=}0]$ for the valuation where $\nu[X{:=}0](x) = 0$ if $x \in X$, and
$\nu[X{:=}0](x) = \nu(x)$ otherwise.
The valuation $\zero \in \V$ is a special valuation such that
$\zero(x) = 0$ for all $x \in \clocks$.
A clock constraint over $\clocks$ is a subset of $\Real^{|\clocks|}$.
We say that a constraint is \emph{rectangular} if it is defined as the
conjunction of a finite set of constraints of the form 
$x  \bowtie k,$  where $k \in \Int$, $x \in \clocks$, and $\bowtie \in \{<,\leq, =,
 >, \geq\}$.    
 For a constraint $g \in \rect(\clocks)$, we write $\sem{g}$ for the set of valuations in
 $\Real^{|\clocks|}$ satisfying the constraint $g$.  
 We write $\rect(\clocks)$ for the set of rectangular constraints over
 $\clocks$.
%
\begin{definition}[Priced Timed Games]
  A turn-based two player \emph{priced timed game} is a tuple
  $\ptg = (\locations_1,\locations_2, L_{init}, \clocks, \trans, \prices,\rgoals)$ where 
  %  \begin{itemize}
  %  \item 
  $\locations_i$ is a finite set of \emph{locations} of Player~$i$, 
  % \item 
  $L_{init} \subseteq L_1 \cup L_2$ is a set of initial locations,
  %  \item 
  $\clocks$ is an (ordered) set of \emph{clocks}, 
  % \item
  $\trans \subseteq \locations \times {\rect}(\clocks)  \times 2^{\clocks}
  \times \locations$ 
  is the \emph{transition relation}, 
  %  \item 
  $\prices \colon \locations \rightarrow \Z$ is the price
  function; and
  %  \item 
  $\rgoals \subseteq \locations$ is the set of target locations.
  % \end{itemize}
\end{definition}

Note that for the sake of simplicity we have omitted the set of actions and location 
invariants from the definition of a PTG (included in definition of PTG in Chapter \ref{chap:ptg}). 
However, all of our results in this chapter hold in the presence of actions and invariants too. 


A priced timed game begins with a token placed on some initial location $\ell$ with  
valuation $\zero$ and cost accumulated being so far being $0$.  
At each round, the player who controls the current location $\ell$ chooses a delay
$t$ (to be elapsed in  $l$) and an outgoing transition $e =(\ell, g, r, \ell') \in
\trans$ to be taken after $t$ delay at $\ell$. 
The clock valuation is then updated according to the delay $t$ and
reset and the cost is incremented by $\prices(\ell) \cdot t$ and the token is moved 
to the location $\ell'$.   
The two players continue moving the token in this fashion, and give rise to a
sequence of locations and transitions called a \emph{play} of the game. 
A configuration or state of a PTG is a tuple $(\ell, \val, \cost)$ where $\ell \in
\locations$ is a location,  $\val \in \V$ is a valuation, and  $\cost$ is the
cost accumulated from the start of play.

W.l.o.g~\cite{BFHLPRV01} we assume that the clock values are bounded : there
exists an constant $M$ such that  $x \leq M$ is satisfied always for all $x \in \clocks$. 

\begin{definition}[PTG semantics]
The semantics of a PTG $\ptg$ is a labelled state-transition game arena 
$\sem{\ptg}$ = $(\nSR = \states_1 \uplus \states_2, S_{init}, A, \nTR)$
where 
\begin{itemize}
\item 
  $\states_j = \locations_j \times \V \times \C$ are the Player~$j$ states with 
  $\nSR = \states_1 \cup \states_2$, 
\item 
  $S_{init} \subseteq \nSR$ are initial states s.t. $(\ell, \nu, c)
  \in S_{init}$ if $\ell \in L_{init}$, $\nu = \zero$ and $c = 0$,
\item 
  $A = \Rplus \times (\locations \times {\rect}(\clocks)  \times 2^{\clocks}
  \times \locations)$ is
  the set of \emph{timed moves}, and 
\item
  $\nTR: \nSR \times A \to \nSR$ is the transition function s.t. 
  for $s = (\ell, \nu, c), s' = (\ell', \nu', c') {\in} \nSR$ and
  $ \tau = (t, e) \in A$ the function $\nTR(s, \tau)$ is defined if $ e = (\ell, g, r,
  \ell')$ is a transition of PTG and $\nu \in \sem{g}$;
  moreover $\nTR(s, \tau) = s'$ if $\nu' = (\nu+t)[r{:=}0]$ and $c' = c + t \cdot
  \prices(\ell)$. We write $s \xrightarrow{\tau} s'$ when $\nTR(s, \tau) = s'$.
\end{itemize}
%% The transition relation is defined as 
%% \begin{enumerate}
%% \item (discrete transition) $(l, \nu, c) \xrightarrow{e} (l', \nu', c')$ if there exists $(l, g,r,l') \in \trans$
%% such that $\nu \models g$, $\nu'=\nu[r{:=}0]$ and $c'=c$,
%% \item (delay transition) $(l, \nu, c) \xrightarrow{t} (l,  \nu',c')$ if 
%% $\nu'=\nu+t$, $c'=c+t\prices(l)$.
%\end{enumerate}
%We define the set of states  and transitions for each player below. 
%\begin{itemize}
%\item 
%\item 
%$\states_j = \locations_j \times \V \times \C$ are the Player~$j$ states, 
%\item $\actions_j = \Rplus \times \trans$ are the actions, 
% \item $goals' = \rgoals \times \V \times \C$
%\item 
%$\trans_j$ is the set of 
%Player~$j$ transitions.
%\end{itemize}
\end{definition}
%% For a  state $(l,\val,\cost)$ a pair $(t,e)$, we have 
%% $(l',\val',\cost')  = \nTR((l,\val,\cost),(t,e))$ iff there is a transition $e=(l,g,a,r,l')$ in $\ptg$ such that 
%% $\val + t \in \sem{g}$, $\val' = \val+t[r:=0]$ and $\cost' = \cost + \prices(l) * t$.

For a state $s = (\ell, \nu, c)$ we write $s(\ell)$, $s(\nu)$ and $s(c)$ for the
location, valuation, and cost of the state. 

A \emph{play} $\rho = \seq{s_0, (t_1, a_1), s_1, (t_2, a_2), \ldots, s_n}$ is a
finite sequence of states and actions s.t.  $s_0 \in S_{init}$ and $s_i
\xrightarrow{(t_{i+1}, a_{i+1})} s_{i+1}$ for all $1 \leq i < n$.
For a finite play $\rho$ we write its last state as $\last(\rho) = s_n$. 
We denote the set of plays as $\runs_{\ptg}$. 
For a play  $\rho = \seq{s_0, (t_1, a_1), s_1, (t_2, a_2), \ldots, s_n}$ we define
$\costp_{\ptg}(\rho) = s_n(c)$.
A \emph{strategy} of player $j$ in $\ptg$ is a function $\strat : \runs_{\ptg}
\to A$ such that for a play $\rho$ the function $\strat(\rho)$  is defined if
$\last(\rho) \in \states_j$.  
We say that a strategy $\strat$ is memoryless if $\strat(\rho) = \strat(\rho')$
when $\left(\last(\rho)(\ell), \last(\rho)(\nu)\right) =
\left(\last(\rho')(\ell), \last(\rho')(\nu)\right)$, otherwise we call it
memoryful. 

We write $\mminstrats$ and $\mmaxstrats$ for the set of strategies of player $1$ and
$2$, respectively. 
A play $\rho$ is said to be \emph{compatible to a strategy} $\strat$ of player
$j \in \set{1, 2}$ if every state $s_i$ in $\rho$ that belongs to Player~$j$,   
$s_{i+1} = \strat(s_i)$. 

Given a pair of strategies $(\sigma_1, \sigma_2) \in \mminstrats \times
\mmaxstrats$, and a state $s$,  the outcome of $(\sigma_1, \sigma_2)$ from
$s$ denoted  $\outcome(s, \strat_1, \strat_2)$ is the unique play that is
compatible with both strategies.  
Given a player $1$ strategy $\sigma_1 \in \mminstrats$ we define its cost
$\costp_{\ptg}(s,\strat_1)$  as 
$\costp_{\ptg}(s,\strat_1) \rmdef \sup_{\strat_2 \in
  \mmaxstrats}(\costp(\outcome(s,\strat_1,\strat_2)))$ . 
%Similarly, we also introduce $\costp_{\ptg}(s,\strat_2)$ as the cost of a Player~2 strategy. 
We now define the  \emph{optimal reachability-cost} for Player~1 from a state
$s$ as 
\[
\optcost{\ptg}(s) = \inf_{\strat_1 \in \mminstrats} \sup_{\strat_2 \in
  \mmaxstrats} (\costp(\outcome(s,\strat_1,\strat_2))).
\]  
A strategy $\strat_1 \in \mminstrats$ is said to be optimal from $s$ if 
$\costp_{\ptg}(s,\strat_1) = \optcost{\ptg}(s)$. 
Since  the optimal strategies may not always exist~\cite{BouLar06} we define the
concept of $\varepsilon$ optimal strategies. 
For $\varepsilon  > 0$ a strategy $\sigma_\varepsilon \in \mminstrats$
is called $\varepsilon-$optimal if  
\[
\optcost{\ptg}(s) \leq \costp_{\ptg}(s,\strat_\varepsilon) < \optcost{\ptg}(s)+\varepsilon.
\] 
The \emph{cost-optmal} reachability problem for PTG asks : given a PTG $\ptg$
and a bound $K \in \Z$ decide whether there exists a strategy for player~1 such
that $\optcost{\ptg}(s) \leq K$ for some starting state $s$. 
The following is a well known result.
\begin{theorem}[\cite{BouBri06}]
  The cost-optimal reachability problem is undecidable for priced timed automata
  with $3$ or more clocks. 
\end{theorem}
\begin{theorem}[\cite{BouLar06,DueIbs13,Rut11}]
\label{thm:1ptg_pat}
  For one-clock priced timed games, the problem of computing
  $\varepsilon$-optimal strategy is decidable.
\end{theorem}



\paragraph{\bf One-Clock PTGs.}

\input{1ptg}


==> termination.tex <==
% \subsection{Complexity and Termination}
 Termination of the Algorithm \ref{algo:optcost_compute} is guaranteed by finiteness of
 $N$, the total number of affine segments that appear in the optcost functions of all locations. 
% The finiteness of $N$ was shown in \cite{BouLar06}. We shall give a brief discussion for the sake 
 %of completeness of our proof. 
 
 Consider a resetfree  FRPTG having $m$ locations.
 Let the  outside cost functions be made of a total of $p$ 
 segments. If $m=1$ then $N = 2p$ as in the worst case, all the $p$ segments could appear in the 
 optcost of the function and each segment could be broken into two pieces, one of which is replaced in 
 Step 3. Now let us define $N$ for $m>1$ locations.  Let $N(m,p)$ denote 
 the total number of line segments when solving for $m$ locations, and considering outside cost functions 
 having $p$ segments. 
  If we are solving for the case $l_{min}$ being a Player~1 location, then 
 $N(m,p) \leq N(m-1, p+ N(1,p + N(m-1,p+1))))$ where 
 the innermost expression $\alpha = N(m-1,p+1)$ corresponds to solving the PTG
 whose locations are indexed by 1
  (locations of the form $(l,1)$ on page 10). 
 This is then used to solve $l_{min}$ which itself could have $p$ segments in the outside cost functions. 
 This gives rise to the expression $\beta = N(1,p + \alpha)$. Finally, this is then used to solve the PTG whose locations are indexed 0. This amounts to $N(m-1, p+\beta)$. 
 
 
 Suppose we are solving for $l_{min}$ being a Player~2 location. 
 We handle this case by making $l_{min}$ urgent and 
 solve the modified PTG $\ptg'$ (where $l_{min}$ is urgent) 
 which has one location less and then uses the 
 computed optcost functions as outside cost functions to solve for $l_{min}$ itself. 
 This can be  repeated as the optcost computed in $\ptg'$ could get updated when the optcost 
 cost of $l_{min}$ itself is computed. This process  gets repeated as many times as the number of 
 segments we started with i.e $p$. Thus the equation is $N(m,p) \leq p . (1 + N(m-1,p+1))$ where 
 $\alpha= N(m-1,p+1)$ is used for solving $\ptg'$, $1 + \alpha$ is used for solving for $l_{min}$ 
 and $p(1+\alpha)$  are the repetitions. 
 
 Solving the above computed equations, yields $N(m,p) \leq 2^{2^{n \cdot 2^n}} \cdot (p+n)^{2^{2^n}}$ which is 
 at most triply exponential. Thus the time needed to compute optimal costs and $\epsilon$-optimal strategies 
 is in $3$-$\exptime$. Now, the additional step we do for RPTG is to transform it into a dwell time 
 PTG and this is polynomial in both space and time. Thus the time needed for RPTG is in $3$-$\exptime$ too. 
 
